On Parameters of Nonlinear Scalar Dynamics from Video: Invariants, Calibration, and Identifiability

Physical parameter estimation from video aims to recover the parameters of a known family of governing dynamical equations from pixel observations. Existing identifiability theory for this setting has focused on linear time-invariant (LTI) second-order systems, leaving open what can be identified for nonlinear scalar dynamics. We develop an identifiability theory for nonlinear scalar second-order ODEs, organized by how their velocity dependence interacts with changes of the learned state coordinate. Under a shared non-collapsed state map and explicit same-state velocity-coverage conditions, we show that parameter identifiability depends on the ODE family: some parameters are uniquely identifiable, while in other families only invariant parameter combinations are identifiable or external physical calibration is required. For laws that are at most linear in velocity, compatibility forces affine coordinate alignment, yielding explicit parameter relations, invariants, and calibration conditions. This affine conclusion extends to broader finite velocity-feature families when coordinate curvature can be separated from the declared velocity dependence. For families admitting a squared-velocity term, nonlinear coordinate ambiguity can remain; a law-derived normalization instead enables affine comparison between canonical laws. Experiments on synthetic systems and real pendulum and free-fall videos support the predicted parameter relations, coverage effects, and calibration requirements.

==> sections/experiments_synthetic.tex <==
\raggedbottom
\section{Synthetic experiments: protocols and supporting results}
\label{app:exp-synth}
The appendix follows the main experiments. Appendix~\ref{app:exp-synth-protocol}
supports Section~\ref{sec:exp-orbit}, including the matched affine-LTI comparison.
Appendices~\ref{app:exp-synth-coverage} and~\ref{app:exp-synth-canonical}
separately support the velocity-coverage and projection experiments in Section~\ref{sec:exp-boundary}.
Each experiment presents observations, data and IC splits, training,
evaluation, and results with discussion in that order.

\subsection{Six-family experiments}
\label{app:exp-synth-protocol}\label{app:exp-synth-orbits}

\subsubsection{Observations, physical systems, and IC collections}
\label{app:exp-synth-observed}

The six-family experiment tests the coordinate and parameter relations of
Section~\ref{sec:scalar-theory}. The five families in Table~\ref{tab:regimes}
are supplemented by the quadratic/Helmholtz family, whose two affine
branches are described in Appendix~\ref{app:helmholtz-branches}.
We simulate each prescribed law at fixed physical coefficients and render
the resulting state trajectories. The angular pendulum is shown as a moving
pendulum; the other families use spring-oscillator renderings
(Figure~\ref{fig:exp-synth-videos}). The simulated states provide evaluation
references and are not coordinate targets for encoder training.


\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/dataset-six-temporal-strips.pdf}
\caption{\textbf{Temporal evolution over two reference oscillation times.}
Nine observations at $0,T/4,\ldots,2T$ show amplitude and timing changes.
Each row starts at a turning point; $T$ is the first interval between
same-type turning points, not an assumed constant period. Damped systems
ring down, whereas Van der Pol approaches a limit cycle.
All frames are $64\times64$.}
\label{fig:exp-synth-videos}
\end{figure}


\begin{table}[H]
\centering\small
\caption{\textbf{Synthetic observations and data splits.} Clip counts are per
IC collection. Each family uses ten collections $\times$ ten optimizer seeds.
Training clips supply images and timestamps for fitting the encoder and law.
Test clips supply the reported held-out errors (coordinate NRMSE
$e_{\rm map}$ (\%)). The permitted coordinate comparison is fitted using
training reference pairs and frozen on test clips.}
\label{tab:exp-synth-data}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lll@{}}
\toprule
Family / experiment & Pixels / Hz / duration & Train / test\\
\midrule
Affine LTI & $64^2$ / 60 / 6 s & 16 / 8\\
Pendulum & $64^2$ / 60 / 8 s & 10 / 4\\
Van der Pol & $64^2$ / 60 / 12 s & 6 / 4\\
Cubic Duffing & $64^2$ / 60 / 8 s & 10 / 4\\
Quintic Duffing & $64^2$ / 60 / 3 s & 16 / 8\\
Quadratic / Helmholtz & $64^2$ / 60 / 8 s & 3 / 4\\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Initial-condition collections.}
For each ODE family, physical coefficients
(Table~\ref{tab:exp-synth-actions}) and the rendering map are fixed.
Table~\ref{tab:exp-synth-initial-states} specifies the nominal initial
position--velocity pairs $(q_0,v_0)$, with $v_0=q'(0)$; the learned
initial value is $z_0=E_\phi(x_0)$ and is not prescribed separately.
Starting from these pairs, ten data seeds generate ten trajectory collections; the different initial conditions
produce different observed video sequences. Each collection contains the
training and test clips listed in Table~\ref{tab:exp-synth-data},
with split assignments inherited from the prescribed trajectory categories.
For the pendulum, initial angles remain fixed and initial angular velocities
receive independent multiplicative perturbations in $[0.95,1.05]$.
For the other five families, initial positions and velocities are perturbed
independently by the same factors.
Each fixed video collection is then fitted with ten optimizer seeds, yielding
$10\times10=100$ fits per family. Data seeds control initial-condition
variation, while optimizer seeds control model initialization and training
sampling.


For experimental plots, write $q$ for physical state and $z=E_\phi(x)$ for
learned state (the theory's $z$ and $\hat z$, respectively), with hats on
learned coefficients. The comparison map is determined by the declared dynamical family.

\begin{table}[H]
\centering\small
\caption{Declared laws, fixed physical coefficients and permitted coordinate actions. Nonzero
$\lambda$ is estimated from training coordinate pairs. The quintic invariant
uses $\beta\ne0$; the plotted physical coefficients are positive.}
\label{tab:exp-synth-actions}
\begin{tabularx}{\linewidth}{@{}p{.40\linewidth}Y@{}}
\toprule
Learned law / physical coefficients & Allowed map / parameter consequence\\
\midrule
$z''+\hat\delta z'+\hat\alpha(z-\hat c)=0$\newline {\footnotesize $(\delta,\alpha,c)=(0.2,4,0)$} &
$z\simeq\lambda q+\tau$; $\hat c\simeq\lambda c+\tau$; $\delta,\alpha$ invariant.\\
$z''+\hat\delta z'+\hat\omega^2\sin z=0$\newline {\footnotesize $(\delta,\omega^2)=(0.15,4)$} &
$z\simeq sq+2\pi n$; $s=\pm1$, $n\in\mathbb Z$; $\delta,\omega^2$ invariant.\\
$z''-\hat\mu(1-z^2)z'+z=0$\newline {\footnotesize $\mu=1.5$} & $z\simeq\pm q$; $\mu$ invariant.\\
$z''+\hat\delta z'+\hat\alpha z+\hat\beta z^3=0$\newline {\footnotesize $(\delta,\alpha,\beta)=(0.2,4,4)$} &
$z\simeq\lambda q$; $\hat\beta\simeq\beta/\lambda^2$;
$\delta,\alpha,\operatorname{sign}\beta$ invariant.\\
$z''+\hat\delta z'+\hat\alpha z+\hat\beta z^3+\hat\gamma z^5=0$\newline {\footnotesize $(\delta,\alpha,\beta,\gamma)=(0.2,4,3,2)$} &
$z\simeq\lambda q$; $\hat\gamma\simeq\gamma/\lambda^4$;
also $\gamma/\beta^2$ invariant.\\
$z''+\hat\delta z'+\hat\alpha z+\hat\beta z^2=0$\newline {\footnotesize $(\delta,\alpha,\beta)=(0.18,1.6,0.8)$} &
Origin: $z\simeq\lambda q$, $\hat\alpha\simeq\alpha$, $\hat\beta\simeq\beta/\lambda$.
Shifted: $z\simeq\lambda(q+\alpha/\beta)$, $\hat\alpha\simeq-\alpha$.\\
\bottomrule
\end{tabularx}
\end{table}

\begin{table}[H]
\centering\small
\caption{\textbf{Nominal initial states before IC perturbation.}
Pairs are $(q_0,v_0)$ in the physical coordinate. Each $\pm$ includes both
signs; in the pendulum row, angle and velocity signs vary independently.
LTI and quintic use the same IC design.}
\label{tab:exp-synth-initial-states}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\linewidth}{@{}p{.17\linewidth}YY@{}}
\toprule
Family & Training pairs & Test pairs\\
\midrule
LTI / quintic &
$(\pm a,0)$, $a\in\{0.25,0.55,0.85,1.15\}$;
$(0,\pm b)$, $b\in\{0.8,1.8,2.8,3.4\}$ &
$(\pm a,0)$, $a\in\{0.65,1.00\}$;
$(0,\pm b)$, $b\in\{0.40,1.00\}$\\
Pendulum &
$(\pm\pi/2,\pi h)$, $h\in\{-1/2,-1/4,0,1/4,1/2\}$ &
$(\pm\pi/2,\pm\pi/8)$\\
Van der Pol &
$(0,\pm0.5)$, $(0,\pm2.5)$, $(\pm3,0)$ &
$(0,\pm1.25)$, $(\pm2.75,0)$\\
Cubic &
$(0,\pm\sqrt{4p^2+2p^4})$,
$p\in\{0.40,0.55,0.70,0.85,1.00\}$ &
$(0,\pm\sqrt{4p^2+2p^4})$,
$p\in\{0.625,0.925\}$\\
Quadratic &
$(0,-1.2)$, $(0,0.8)$, $(0,1.2)$ &
$(-0.4,0.65)$, $(0.4,-0.65)$,
$(-0.15,1.0)$, $(0.15,-1.0)$\\
\bottomrule
\end{tabularx}
\end{table}

\subsubsection{Training and evaluation}
\label{app:exp-synth-training-details}\label{app:exp-synth-evaluation}

LTI, cubic, quintic and quadratic use per-frame CNNs with three convolutional
blocks (base width 32), GroupNorm, GELU, a 128-unit MLP and a scalar output.
Inputs are $64\times64$; cubic frames use Lanczos resizing.
The encoder and dynamical coefficients are optimized jointly. The
$\mathcal L_{\mathrm{var}}$ penalty introduced in Section~\ref{sec:setup} uses the
standard-deviation threshold $s_{\mathrm{floor}}=0.02$
(Eq.~\ref{eq:AB_variance_floor}). Table~\ref{tab:exp-synth-training}
lists the optimization settings for all six families.
The pendulum and Van der Pol scalar output biases are initialized in
$[-3\pi,3\pi]$ and $[-0.5,0.5]$, respectively.

\begin{table}[H]
\centering\small
\caption{\textbf{Training settings for the six-family experiment.}
All use Adam and the final checkpoint after the stated number of updates
(optimizer steps). Learning rates are encoder / dynamical law.
Each family has 100 fits.}
\label{tab:exp-synth-training}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lcccc@{}}
\toprule
Family & IC collections & Seeds per set & Updates & $\mathrm{lr}_{\mathrm{enc}}/\mathrm{lr}_{\mathrm{ode}}$\\
\midrule
Affine LTI & 10 & 10 & 2,000 & $0.0005/0.003$\\
Pendulum & 10 & 10 & 2,500 & $0.001/0.005$\\
Van der Pol & 10 & 10 & 5,000 & $0.001/0.003$\\
Cubic Duffing & 10 & 10 & 8,000 & $0.0005/0.1$\\
Quintic Duffing & 10 & 10 & 8,000 & $0.0005/0.003$\\
Quadratic / Helmholtz & 10 & 10 & 6,000 & $0.0005/0.003$\\
\bottomrule
\end{tabular}
\end{table}

\noindent\textbf{Coordinate alignment and parameter comparison.}
After training, freeze the encoder and fitted law. Estimate the
family-permitted map $\hat f$ from training reference pairs $(q,z)$:
LTI uses an affine least-squares map, the pendulum selects a sign and
$2\pi$ shift, and Van der Pol selects a sign. Cubic and quintic use
$\lambda=\sum qz/\sum q^2$. Quadratic fits both permitted branches on
training data and freezes the branch and scale with the smaller coordinate
error (Table~\ref{tab:exp-synth-actions}). No test states are used to
select or refit this map.

On test clips, set $x=q$ and $\widetilde x=\hat f^{-1}(z)$ in
Eq.~\eqref{eq:common-coordinate-error}: compute coordinate NRMSE within
each clip and take the clip median to obtain one $e_{\rm map}$ per fit.
For parameter evaluation, transform the physical law with the same frozen
map and branch to obtain $\theta^{\rm ref}$. Equation~\eqref{eq:common-parameter-error}
then gives $e_\theta$ as the largest relative error over the listed nonzero
dynamical coefficients, retaining coefficient signs and excluding the
LTI equilibrium. Thus the coordinate and parameter checks test the same
predicted relation, rather than choosing a scale from coefficient ratios.
The 100 per-fit errors are summarized using the conventions in
Appendix~\ref{app:metric-conventions}; the acceleration comparison below
uses $e_{\rm dyn}$ from Eq.~\eqref{eq:common-dynamics-error}.

\subsubsection{Results and discussion}

Figure~\ref{fig:exp-orbit} shows the learned coefficients and coordinate
maps. Table~\ref{tab:app-exp-synth-cohort} summarizes the 100 fits per family;
Figures~\ref{fig:exp-synth-errors} and~\ref{fig:exp-synth-orbit-by-ic}
separate these fits by IC collection, showing the ten optimizer seeds
within each collection.



\begin{table}[H]
\centering\small
\caption{\textbf{Parameter relative error and coordinate recovery.}
Percentages are median [Q25, Q75] over all 100 fits per family.}
\label{tab:app-exp-synth-cohort}
\begin{tabular}{@{}lcc@{}}
\toprule
Family (100 fits) & Parameter $e_\theta$ (\%) & Coordinate $e_{\rm map}$ (\%)\\
\midrule
Affine LTI & 0.85 [0.52, 1.65] & 1.68 [1.53, 1.90]\\
Pendulum & 1.44 [0.84, 2.17] & 3.58 [2.27, 5.99]\\
Van der Pol & 0.31 [0.13, 0.61] & 2.45 [1.69, 3.71]\\
Cubic & 2.56 [1.60, 4.60] & 0.82 [0.68, 1.08]\\
Quintic & 1.68 [1.02, 2.29] & 0.78 [0.62, 1.06]\\
Quadratic & 2.47 [1.31, 4.37] & 3.29 [1.96, 6.08]\\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/synthetic-ic-coordinate.pdf}
\caption{\textbf{Test coordinate NRMSE $e_{\rm map}$ by IC collection.}
Each family contains ten IC collections, each with ten optimizer seeds.
Dots show $e_{\rm map}$; black bars
give each collection's median and interquartile range.
Colors match Figure~\ref{fig:exp-orbit};
IC indices are local to each family. The logarithmic vertical limits vary
by family.}
\label{fig:exp-synth-errors}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/synthetic-ic-orbit.pdf}
\caption{\textbf{Parameter relative error $e_\theta$ by IC collection.}
The same fits and IC groups as in Figure~\ref{fig:exp-synth-errors}, now
showing $e_\theta$.
Within each group, horizontal offsets follow optimizer-seed order and
are identical in both figures. Bars show median and interquartile range.}
\label{fig:exp-synth-orbit-by-ic}
\end{figure}

Median parameter relative errors range from $0.31\%$ to $2.56\%$.
Cubic and quintic combine sub-$1\%$ median coordinate NRMSE with the
predicted $\beta/\gamma$ scaling in Figure~\ref{fig:exp-orbit}.
Pendulum and Van der Pol have median coordinate errors of $3.58\%/2.45\%$
and parameter errors of $1.44\%/0.31\%$.
The IC breakdown shows both variation across trajectory collections and
the spread across optimizer seeds within each collection.
These comparisons assess finite-data agreement with the family-specific
relations. Proposition~\ref{prop:affine-realizability} constructs exact
alternative encoders under representability and affine-closure assumptions;
the empirical errors do not certify these assumptions or every continuous-time
premise (Appendix~\ref{app:operational-details}).

\subsubsection{Matched affine-LTI comparison}
\label{app:exp-synth-adequacy}

This experiment probes the scope of affine-LTI modeling and the loss in
dynamical accuracy caused by ODE-family misspecification. We keep the
observations and ICs unchanged, train the encoder jointly with an affine-LTI
law, and then evaluate the fitted coefficients on trajectories from the
held-out test videos. The affine-LTI dataset provides a matched-family
control, while the five nonlinear datasets test the cost of restricting
the learned dynamics to this family.
For each of the six families, we pair the 100 fitted models with 100
affine-LTI controls, $z''+\hat\delta z'+\hat\alpha(z-\hat c)=0$.
Each pair shares the video data, encoder architecture and initial weights,
training-window sampling, optimizer settings, and update budget
(Table~\ref{tab:exp-synth-training}); the LTI equilibrium $\hat c$ is learned
jointly. Pairing covers ten IC collections and ten optimizer seeds per family.

\paragraph{Physical-acceleration comparison.}
For each model, fit $z\simeq\lambda q+\tau$ on training frames and freeze
it on test trajectories. Evaluate $e_{\rm dyn}$ using the stored physical
states and derivatives, with
\[
 \widetilde F=\lambda^{-1}\hat F(\lambda q+\tau,\lambda q'),
 \qquad F=q''.
\]
Here $\hat F$ uses the fitted coefficients without refitting on test
data. Equation~\eqref{eq:common-dynamics-error} measures how accurately
the learned dynamical law reproduces physical acceleration along the
held-out trajectories, including the effect of family misspecification;
it does not integrate a rollout or compare coefficients from different
families. The LTI oracle fits acceleration directly to $(q,q',1)$ on training trajectories
with the matching coefficient-sign constraints and uses the same test
comparison. Wins count paired fits with lower $e_{\rm dyn}$ for the
declared family model.

\begingroup
\setlength{\intextsep}{6pt}
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/family-adequacy-ic-six.pdf}
\caption{\textbf{Matched affine-LTI comparison across IC collections.}
Each family has ten IC collections and ten paired optimizer seeds per
collection. Faint lines show individual seeds; solid curves and bands give
the within-IC median and interquartile range of $e_{\rm dyn}$.
Dashed curves show the training-fitted physical-state LTI oracle.
Both methods in A use the affine-LTI family.}
\label{fig:app-exp-synth-adequacy}
\end{figure}

\begin{table}[H]
\centering\small
\caption{\textbf{Test acceleration relative RMSE.} Median [Q25, Q75]
percentages over 100 pairs per family. Wins count pairs with a smaller
$e_{\rm dyn}$ for the declared family model.}
\label{tab:exp-matched-lti}
\begin{tabular}{@{}lccc@{}}
\toprule
Dataset & Affine LTI (\%) & Family model (\%) & Family wins\\
\midrule
Affine LTI & 3.86 [1.96, 6.58] & 4.56 [2.16, 6.84] & 46/100\\
Pendulum & 11.34 [11.20, 11.70] & 2.17 [1.43, 3.89] & 99/100\\
Van der Pol & 88.48 [88.01, 88.79] & 5.80 [3.07, 9.21] & 98/100\\
Cubic & 17.92 [17.46, 18.53] & 0.81 [0.57, 1.39] & 100/100\\
Quintic & 24.29 [23.46, 25.02] & 0.54 [0.33, 0.89] & 100/100\\
Quadratic & 22.03 [20.42, 23.85] & 3.15 [1.70, 6.68] & 92/100\\
\bottomrule
\end{tabular}
\end{table}
\endgroup

Across the five nonlinear datasets, the declared family has lower median
acceleration error in all ten IC collections and wins 92--100 of the 100
individual pairs. On the affine-LTI dataset, the two fits have comparable
error distributions.

\FloatBarrier
\subsection{Coverage}
\label{app:exp-synth-coverage}\label{app:exp-synth-observations}

\subsubsection{Observations, physical system, and IC collections}
\label{app:exp-synth-coverage-setup}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth,trim=0 76 0 30,clip]{figures/experiments/boundary-video-strips.pdf}
\caption{Opposite odd-drag crossings. Both rows show $96\times96$ inputs
at 60 Hz, aligned at the same position at $t=0$. The central frames have
the same geometry despite opposite velocities; labels give time in seconds.}
\label{fig:exp-boundary-videos}
\end{figure}


The physical system is
$q''=-kq-\delta q'-\kappa q'|q'|$, with spring coefficient $k=0.8$,
linear damping $\delta=0.18$, and quadratic drag $\kappa=0.22$.
Each IC collection contains 24 training and eight test clips of 1 s,
rendered at $96\times96$ pixels and 60 Hz (61 frames).

\noindent\textbf{Theoretical expectation.}
The experiment tests the curvature-column exclusion in
Theorem~\ref{thm:feature-separation}. A nonlinear coordinate map contributes
$f''(q)v^2$ to the acceleration. Although $v|v|$ differs from $v^2$ over
two-way motion, these columns coincide for positive velocities (and differ
only by sign for negative velocities). One-way motion therefore cannot
separate drag from coordinate curvature, regardless of the number of
speeds. With two directions and two distinct speed magnitudes, the
augmented feature matrix $[1,v,v|v|,v^2]$ has rank four, giving the
theorem's raw-affine conclusion under its remaining assumptions.
The corresponding drag relation is $c_d=-\kappa/|\lambda|$
(Eq.~\eqref{eq:exp-coverage-orbit}). The test is whether this change in
coverage improves parameter recovery even when coordinate errors are small.

We vary the number $K$ of speed magnitudes and whether trajectories cross
$q=0$ in one or both directions. As in Appendix~\ref{app:exp-synth-protocol},
an \emph{IC collection} groups videos generated from one prescribed set
of physical trajectory conditions. Here the conditions are the crossing
velocities at $q=0$, which determine the simulated trajectories.
Ten data seeds independently perturb
the base magnitudes $\{0.8,1.35,1.95\}$ by factors in $[0.97,1.03]$.
One-way $K=1$ uses the middle magnitude; $K=3$ uses all three;
$K=6$ uses six values spanning the same envelope. Two-way $K=1$ uses
both signs of the middle magnitude; $K=2$ uses both signs of the smallest
and largest magnitudes; $K=3$ uses all three. Appearance repetitions give
24 training clips in every condition. The test pools use crossing speeds
near $\{1.1,1.7\}$ for one-way designs and $\{-1.1,1.1\}$ for two-way
designs. Evaluation below uses the four positive-direction test clips
near $1.1$ shared by all six conditions within each IC collection.

\subsubsection{Training and evaluation}
\label{app:exp-synth-coverage-training}

Each of the ten IC collections is crossed with five optimizer seeds, giving 50 fits per
condition. A spatial soft-argmax encoder is followed by a learned cubic
polynomial head. It is jointly fitted with
$z''=c_0(z)+c_1(z)z'+c_d(z)z'|z'|$, where the polynomial degrees of
$(c_0,c_1,c_d)$ are $(5,3,5)$. Derivatives use a 31-frame, degree-two
local-polynomial fit. Table~\ref{tab:exp-coverage-training} gives the
optimization settings; evaluation uses the final checkpoint.

\begin{table}[H]
\centering\small
\caption{\textbf{Coverage training settings.} Adam; each coverage condition uses ten IC collections and five optimizer seeds per collection.}
\label{tab:exp-coverage-training}
\begin{tabular}{@{}cccc@{}}
\toprule
IC collections & Seeds per collection & Updates & $\mathrm{lr}_{\mathrm{enc}}/\mathrm{lr}_{\mathrm{ode}}$\\
\midrule
10 & 5 & 5,000 & $0.0005/0.002$\\
\bottomrule
\end{tabular}
\end{table}


\paragraph{Coordinate comparison.}
Fit $z\simeq\lambda q+\tau$ on training references, then use $x=q$ and
$\widetilde x=(z-\tau)/\lambda$ in Eq.~\eqref{eq:common-coordinate-error}
to compute $e_{\rm map}$. Each clip contributes its frames with
$q\in[-0.2,0.2]$; all six conditions use the same four test clips within
each IC collection.

\paragraph{Parameter relative error for the mean drag coefficient.}
Substitution of $z=\lambda q+\tau$ into the physical law gives
\begin{equation}
 c_0(z)=-k(z-\tau),\qquad c_1(z)=-\delta,\qquad
 c_d(z)=-\frac{\kappa}{|\lambda|}.
 \label{eq:exp-coverage-orbit}
\end{equation}
Let $\bar\kappa=-\operatorname{mean}c_d$ be the mean learned drag
magnitude, evaluated on 101 equally spaced learned-coordinate values
over the encoded training interval $q\in[-0.2,0.2]$.
The parameter comparison uses the scale-corrected mean
$\widehat\kappa_{\mathrm{aligned}}=|\lambda|\bar\kappa$ against
$\kappa=0.22$ in Eq.~\eqref{eq:common-parameter-error}, with
the same training-fitted $\lambda$ as the coordinate
comparison. Figure~\ref{fig:exp-coverage-orbit} shows both errors for all
six designs.

\paragraph{Velocity-feature rank.}
The feature rank concerns $[1,v,v|v|,v^2]$
(Section~\ref{subsec:feature-separation}). It is evaluated at 21 shared
positions in $[-0.2,0.2]$, using the distinct velocities at each position;
Figure~\ref{fig:exp-coverage-orbit}A reports the minimum rank. Rank four separates the declared features from the curvature column.
A smaller rank fails this sufficient condition; it does not by itself
establish nonidentifiability of every parameter.

\subsubsection{Results and discussion}
\label{app:exp-synth-coverage-results}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/coverage-six-errors.pdf}
\caption{\textbf{Velocity coverage, parameter recovery, and coordinate accuracy.}
A: minimum rank of $[1,v,v|v|,v^2]$ over 21 shared positions in
$[-0.2,0.2]$; all ten IC collections give the displayed rank for each condition.
The dashed line marks full rank. B: coordinate NRMSE $e_{\rm map}$
(Eq.~\eqref{eq:common-coordinate-error}) on the same four test clips
within each IC collection. C: parameter relative error $e_\theta$ of the
scale-corrected mean drag coefficient (Eq.~\eqref{eq:common-parameter-error}).
B/C show all 50 fits per condition, colored by IC collection, with matching
horizontal offsets. Black bars show the median and interquartile range
over the 50 fits, using the convention of Figures~\ref{fig:exp-synth-errors}
and~\ref{fig:exp-synth-orbit-by-ic}; numbers give medians (\%).
All axes are linear. $K$ counts speed magnitudes.}
\label{fig:exp-coverage-orbit}
\end{figure}

One-way motion gives $v|v|=v^2$, so adding speeds does not separate the
drag feature from the curvature term introduced by a nonlinear coordinate
map. Median drag-parameter errors are $43.68\%$ and $44.97\%$ for
one-way $K=3,6$, compared with $1.34\%$ and $1.25\%$ for two-way
$K=2,3$, which have full feature rank. Median coordinate NRMSE is
$1.07$--$1.44\%$ across all six conditions. Accurate coordinates therefore
coexist with substantial errors in the recovered mean drag coefficient
when velocity coverage is insufficient.

\FloatBarrier
\subsection{Normalization}
\label{app:exp-synth-canonical}

\subsubsection{Observations, projected dynamics, and IC collections}
\label{app:exp-synth-canonical-setup}

We simulate a pendulum with angular dynamics
$q''+0.15q'+4\sin q=0$, released from rest at different initial angles.
An orthographic camera looks along the vertical axis and records
$y=\sin q$ on $|q|<\pi/2$, discarding the depth coordinate
(Figure~\ref{fig:exp-projection-geometry}). The projected rod and bob are
rendered as $96\times96$ grayscale frames. Thus the observation depends
nonlinearly on the physical angle even before learning.

\begin{figure}[H]
\centering
\includegraphics[width=.82\linewidth]{figures/experiments/projection-geometry.pdf}
\par\smallskip
\includegraphics[width=\linewidth,trim=0 0 0 173,clip]{figures/experiments/boundary-video-strips.pdf}
\caption{\textbf{Projected pendulum observations.}
An orthographic camera looks along the vertical axis, retaining
$X=L\sin q$ and discarding the depth coordinate $-L\cos q$.
The projected rod and constant-size bob produce the image coordinate
$y=\sin q$. Bottom: nine $96\times96$ observations from $0$ to $3T/2$
for a $70^\circ$ release; $T$ is the first full oscillation duration.
The illustrative strip continues the original ODE and renderer beyond
the 4.8 s training-clip duration.}
\label{fig:exp-projection-geometry}
\end{figure}

\noindent\textbf{Projected law and theoretical expectation.}
Differentiating $y=\sin q$ introduces the squared-velocity coefficient
$-y/(1-y^2)$ into the projected law. We fit the corresponding structured family in a learned
coordinate with free scale $s>0$ and offset $b$:
\begin{equation}
 z''=-\delta z'-\omega^2(z-b)\sqrt{1-u^2}
 -\rho\frac{z-b}{s^2-(z-b)^2}(z')^2,\qquad u=\frac{z-b}{s}.
 \label{eq:app-exp-synth-projected-law}
\end{equation}
Here $\rho$ controls the squared-velocity channel. The exact projected
law $z=s\sin q+b$ has $(\delta,\omega^2,\rho)=(0.15,4,1)$.
This experiment tests Section~\ref{sec:connection-boundary}: a squared-velocity
channel permits nonlinear coordinate changes, while canonical normalization
restores an affine comparison between the transformed laws.
The normalizer in Eq.~\eqref{eq:exp-projection-normalizer} removes that
channel and becomes $s\arcsin((z-b)/s)$ when $\rho=1$.
Because the angular law itself has no squared-velocity term, its canonical
coordinate is $q$; Theorem~\ref{thm:canonical-report-orbit} therefore predicts
one shared affine relation $\psi(z)\simeq\lambda q+\tau$.
We expect this correction to reduce angular distortion and to recover
the angular restoring force and damping. The comparison applies on the
regular chart $|z-b|<s$ and requires at least three distinct physical
velocities at each covered position for this degree-two velocity family.

\noindent\textbf{IC collections and the coordinate comparison.}
We use two data regimes, identified by their maximum
training release angles of $70^\circ$ and $85^\circ$
(Table~\ref{tab:exp-normalization-data}). Within each regime, all training
angles contribute trajectories to a single encoder and dynamical law;
test trajectories start from distinct release angles. Multiple release
angles sample different velocities at shared positions, addressing
the theorem's coverage requirement.

\begin{table}[H]
\centering\small
\caption{\textbf{Release-angle sets and video counts for normalization.}
Angles are nominal initial conditions in degrees. Counts are per IC
collection, with four appearance repetitions per angle.}
\label{tab:exp-normalization-data}
\begin{tabular}{@{}lccc@{}}
\toprule
Max. train angle & Training angles & Test angles & Train / test clips\\
\midrule
$70^\circ$ & $30,45,60,70$ & $40,55,65$ & $16/12$\\
$85^\circ$ & $30,45,60,70,80,85$ & $40,55,65,75,82$ & $24/20$\\
\bottomrule
\end{tabular}
\end{table}

In each regime, ten data seeds generate ten IC collections by
perturbing nonmaximal training angles by $\pm1.5^\circ$ and test angles
by $\pm1^\circ$; the maximum training angle stays fixed. An IC
collection contains the resulting training and test release trajectories;
IC indices 1--10 enumerate these data seeds within each regime.
Each trajectory has four renderings with appearance variation.
Clips use $96\times96$ frames and last 4.8 s at 30 Hz (145 frames).
Both regimes remain within $|q|<90^\circ$; the inverse projection
sensitivity $1/\cos q$ at the training-range endpoints is 2.9 and 11.5,
respectively. In each regime, raw and canonical coordinates are evaluated
on the same held-out videos.

Figure~\ref{fig:exp-normalization-residuals} illustrates the coordinate
correction tested here: affine alignment of the raw coordinate leaves
angle-dependent residuals, whereas alignment after normalization reduces
them. Both comparisons use the same test videos and training-fitted
alignment maps; the fitting procedure and $e_{\rm map}$ are specified in
Appendix~\ref{app:exp-synth-canonical-training}.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/normalization-coordinate-residuals.pdf}
\caption{\textbf{Canonical normalization removes the systematic coordinate distortion.}
Test-angle residuals after training-fitted affine alignment. Thin curves
show individual fits; thick curves and shading show pointwise medians and
interquartile ranges. Each panel uses 50 raw fits and 50/49 canonical fits.
Binning is for display; $e_{\rm map}$ in Table~\ref{tab:exp-normalization}
uses the original test frames (Eq.~\eqref{eq:common-coordinate-error}).}
\label{fig:exp-normalization-residuals}
\end{figure}

\subsubsection{Training and evaluation}
\label{app:exp-synth-canonical-training}

Jointly fit the spatial soft-argmax encoder and the structured law in
Eq.~\eqref{eq:app-exp-synth-projected-law}.
Initialize $(\delta,\omega^2,\rho,s,b)=(0.12,3.2,0.8,0.82,0)$.
Each IC collection is trained with five optimizer seeds, giving 50 fits per regime. Training samples
four 97-frame windows per step and uses 21-frame, degree-four
local-polynomial derivatives. The standard-deviation threshold is
$s_{\mathrm{floor}}=0.03$ (Eq.~\ref{eq:AB_variance_floor});
the variance and chart penalties have weight 100, with the latter applied
outside $|u|\le0.985$.

\begin{table}[H]
\centering\small
\caption{\textbf{Normalization training settings.} Adam; each release-angle regime uses ten IC collections and five optimizer seeds per collection.}
\label{tab:exp-normalization-training}
\begin{tabular}{@{}cccc@{}}
\toprule
IC collections & Seeds per collection & Updates & $\mathrm{lr}_{\mathrm{enc}}/\mathrm{lr}_{\mathrm{ode}}$\\
\midrule
10 & 5 & 6,000 & $0.0002/0.002$\\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Coordinate normalization and NRMSE.}
After training, freeze the encoder and law and apply the canonical branch of
Figure~\ref{fig:nonlinear-training-pipeline}; this step requires no physical
anchors.
The fitted quadratic-velocity coefficient is
$c_2(w)=-\rho(w-b)/[s^2-(w-b)^2]$.
Solving \eqref{eq:normalizer-ode} with $\psi(b)=0$ and $\psi'(b)=1$ gives
\begin{equation}
 \psi(z)=s\int_0^{(z-b)/s}(1-u^2)^{-\rho/2}\,du.
 \label{eq:exp-projection-normalizer}
\end{equation}
For $\rho=1$, this becomes $s\arcsin((z-b)/s)$.
For each fitted model, evaluate the integral using its learned
$(\rho,s,b)$. For $h(z)=z$ or $\psi(z)$, fit
$h(z)\simeq a_hq+b_h$ on training references and set
$\widetilde q=[h(z)-b_h]/a_h$ on test clips.
Set $x=q$ and $\widetilde x=\widetilde q$ in
Eq.~\eqref{eq:common-coordinate-error}; compute NRMSE within each test
clip and then take the clip median for $e_{\rm map}$.
Residual curves show $\widetilde q-q$
as a function of angle, exposing systematic distortion that a scalar
NRMSE summarizes.

\paragraph{Numerical implementation.}
The integral is evaluated by cumulative trapezoidal quadrature with 40,001
integration nodes spanning the encoded training/test values and the basepoint $b$.
A \emph{defined map} requires $s^2-(z-b)^2>0$ throughout
this interval, so that the real-valued normalizer is regular from its
basepoint to every evaluation state. All 50 fits in the $70^\circ$ regime
pass this check. One $85^\circ$ fit violates it, leaving 49 defined
canonical maps (Table~\ref{tab:exp-normalization}); the raw-coordinate
statistics still include all 50 fits.

\paragraph{Physical parameters and the transformed law.}
Report the individual parameter relative errors $e_{\theta,j}$ from
\eqref{eq:common-parameter-error} for the physical coefficients
$(\delta,\omega^2)$ and the quadratic-velocity factor $\rho$ against
$(0.15,4,1)$. Let $A(z)$ and $B(z)$ be the velocity-independent and
linear-velocity channels in \eqref{eq:app-exp-synth-projected-law}.
Using the training comparison $\psi(z)\simeq\lambda q+\tau$, evaluate
\[
 z_q=\psi^{-1}(\lambda q+\tau),\qquad
 F_q(q)=\psi'(z_q)A(z_q)/\lambda,\qquad D_q(q)=B(z_q).
\]
Compare $F_q$ with $-4\sin q$ and $D_q$ with $-0.15$ on 361 points
in the common interior $[-0.9,0.9]$ rad, using $e_{\rm dyn}$ for each
channel (Eq.~\eqref{eq:common-dynamics-error}). These comparisons test whether normalization recovers the
angular restoring force and damping across the common state interval.

\subsubsection{Results and discussion}
\label{app:exp-synth-canonical-results}

Normalization reduces the coordinate distortion in
Figure~\ref{fig:exp-normalization-residuals} and lowers median test NRMSE
from $5.66\%$ to $0.29\%$ at $70^\circ$ and from $8.19\%$ to $0.34\%$
at $85^\circ$ (Table~\ref{tab:exp-normalization}).
Across the 49 paired $85^\circ$ fits with defined maps, the within-fit
reduction is 7.87 [7.70, 8.02] percentage points. Median $\omega^2$
errors below $0.15\%$ (Table~\ref{tab:app-exp-synth-canonical}) and
restoring-force error near $0.19\%$ connect
this improved coordinate recovery to agreement with the physical dynamics.
Figure~\ref{fig:exp-canonical-law} separates the two release-angle regimes
and resolves variation across IC collections and optimizer seeds.
Force-error medians vary across IC collections despite similar pooled
errors in the two regimes.

\begin{table}[H]
\centering\small
\caption{\textbf{Fitted law coefficients.} Parameter relative errors $e_{\theta,j}$
(\%), median [Q25, Q75] over all 50 fits per support, against
$(\delta,\omega^2,\rho)=(0.15,4,1)$.}
\label{tab:app-exp-synth-canonical}
\begin{tabular}{@{}lccc@{}}
\toprule
Max. train angle & $\delta$ error & $\omega^2$ error & $\rho$ error\\
\midrule
$70^\circ$ & 0.80 [0.51, 1.04] & 0.11 [0.05, 0.15] & 1.58 [0.94, 1.74]\\
$85^\circ$ & 1.16 [0.97, 1.43] & 0.14 [0.06, 0.21] & 1.66 [1.27, 1.85]\\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/experiments/canonical-law-check.pdf}
\caption{\textbf{Restoring force and damping after normalization.}
Rows separate the $70^\circ$ and $85^\circ$ regimes, with identical axis
ranges for corresponding panels. A, D: force residuals
$100(F_q-F)/\mathrm{RMS}(F)$, where $F=-4\sin q$; thin curves show
individual fits, and thick curves and shading show pointwise medians and
interquartile ranges, as in Figure~\ref{fig:exp-normalization-residuals}.
B, E: restoring-force relative RMSE; C, F: damping relative RMSE $e_{\rm dyn}$
(Eq.~\eqref{eq:common-dynamics-error}) by IC collection; each point is
one optimizer seed, and black bars show the median and interquartile range.
There are five defined maps per IC collection except IC 7 at $85^\circ$
(marked $*$), which has four.
Restoring-force relative RMSEs are $0.190\%$ [0.149, 0.232] and $0.193\%$ [0.172, 0.231] for the $70^\circ$
and $85^\circ$ supports, respectively (median [Q25, Q75]).}
\label{fig:exp-canonical-law}
\end{figure}

\flushbottom


==> sections/operational.tex <==
\paragraph{Interpreting the empirical comparisons.}
The experiments distinguish invariant quantities, family-allowed coordinate
and coefficient alignments, and physical-unit estimates after external
calibration. Each comparison is relative to its declared family, parameter
stratum, and remaining branches. Appendix~\ref{app:operational-details}
collects the assumptions and diagnostics needed to interpret these reports;
finite-data checks provide evidence about the premises of the theory.

